Automatic Face Image Quality Prediction

Face image quality can be defined as a measure of the utility of a face image to automatic face recognition. In this work, we propose (and compare) two methods for automatic face image quality based on target face quality values from (i) human assessments of face image quality (matcher-independent), and (ii) quality values computed from similarity scores (matcher-dependent). A support vector regression model trained on face features extracted using a deep convolutional neural network (ConvNet) is used to predict the quality of a face image. The proposed methods are evaluated on two unconstrained face image databases, LFW and IJB-A, which both contain facial variations with multiple quality factors. Evaluation of the proposed automatic face image quality measures shows we are able to reduce the FNMR at 1% FMR by at least 13% for two face matchers (a COTS matcher and a ConvNet matcher) by using the proposed face quality to select subsets of face images and video frames for matching templates (i.e., multiple faces per subject) in the IJB-A protocol. To our knowledge, this is the first work to utilize human assessments of face image quality in designing a predictor of unconstrained face quality that is shown to be effective in cross-database evaluation.

==> biography/biography.tex <==
% biography section
\begin{biography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Phos/Lacey}}]{Lacey Best-Rowden} received her B.S. degree in ...[Placeholder] She is a student member of the IEEE.
\end{biography}

\begin{biography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Phos/Hu}}]{Hu Han} is a Research Associate in the Department of Computer Science and Engineering at Michigan State University, East Lansing. He received the B.S. degree in Computer Science from the Shandong University, Jinan, China, in 2005 and the Ph.D. degree from the Institute of Computing Technology, Chinese Academy of Sciences, Beijing, China, in 2011. His research interests include computer vision, pattern recognition, and image processing, with applications to biometrics, forensics, law enforcement, and security systems. He is a member of the IEEE.
\end{biography}

\begin{biography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Phos/Charles}}]{Charles Otto} received his B.S. degree in the Department of Computer Science and Engineering at Michigan State University in 2008. He was a research engineer at IBM in 2006-2011. Since 2012, he has been working toward the Ph.D. degree in the Department of Computer Science and Engineering at Michigan State University. His research interests include pattern recognition, image processing, and computer vision, with applications to face recognition.
\end{biography}


\begin{biography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Phos/Brendan}}]{Brendan F. Klare} received the B.S. and M.S. degrees in computer science from the University of South Florida in 2007 and 2008, respectively, and the Ph.D. degree in computer science from Michigan State University in 2012. He is a lead scientist at Noblis. From 2001 to 2005, he served as an airborne ranger infantryman in the 75th Ranger Regiment. His research interests include pattern recognition, image processing, and computer vision. He has authored several papers on the topic of face recognition, and he received the Honeywell Best Student Paper Award at the 2010 IEEE Conference on Biometrics: Theory, Applications, and Systems (BTAS). He is a member of the IEEE.
\end{biography}

\begin{biography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Phos/Anil}}]{Anil K. Jain} is a university distinguished professor in the Department of Computer Science and Engineering at Michigan State University, East Lansing. His research interests include pattern recognition and biometric authentication. He served as the editor-in-chief of the \uppercase{IEEE Transactions on Pattern Analysis and Machine Intelligence} (1991-1994). He is the coauthor of a number of books, including Handbook of Fingerprint Recognition (2009), Handbook of Biometrics (2007), Handbook of Multibiometrics (2006), Handbook of Face Recognition (2005), BIOMETRICS: Personal Identification in Networked Society (1999), and Algorithms for Clustering Data (1988). He served as a member of the Defense Science Board and The National Academies committees on Whither Biometrics and Improvised Explosive Devices. He received the 1996 \uppercase{IEEE Transactions on Neural Networks} Outstanding Paper Award and the Pattern Recognition Society best paper awards in 1987, 1991, and 2005. He has received Fulbright, Guggenheim, Alexander von Humboldt, IEEE Computer Society Technical Achievement, IEEE Wallace McDowell, ICDM Research Contributions, and IAPR King-Sun Fu awards. He is a fellow of the AAAS, ACM, IAPR, SPIE, and IEEE.
\end{biography}

